Nowhere to Hide: Cross-modal Identity Leakage between Biometrics and Devices

Along with the benefits of Internet of Things (IoT) come potential privacy risks, since billions of the connected devices are granted permission to track information about their users and communicate it to other parties over the Internet. Of particular interest to the adversary is the user identity which constantly plays an important role in launching attacks. While the exposure of a certain type of physical biometrics or device identity is extensively studied, the compound effect of leakage from both sides remains unknown in multi-modal sensing environments. In this work, we explore the feasibility of the compound identity leakage across cyber-physical spaces and unveil that co-located smart device IDs (e.g., smartphone MAC addresses) and physical biometrics (e.g., facial/vocal samples) are side channels to each other. It is demonstrated that our method is robust to various observation noise in the wild and an attacker can comprehensively profile victims in multi-dimension with nearly zero analysis effort. Two real-world experiments on different biometrics and device IDs show that the presented approach can compromise more than 70\% of device IDs and harvests multiple biometric clusters with ~94% purity at the same time.

==> section/cross_labeling.tex <==
%!TEX root = ../autotune.tex
\section{Cross-modality Labeling} % (fold)
\label{sec:cross_modality_labeling}

In this section, we introduce the labeling module in {\sysname}. The challenge in this module is that collected facial images and sniffed WiFi data are temporally unaligned. For example, detecting a device WiFi address does not imply that the device owner will be captured by the camera at the exact instant and vice versa. Such mismatches in cross-modality data distinguish our problem from prior sensor fusion problems, where both multiple sensors are observing a temporal evolving system. In order to tackle the above challenge, we leverage the diverse attendance patterns in events and use a two-step procedure in isolated. Images $\mathcal{X}$ are firstly grouped together into clusters across all sessions, and we then associate clusters with device IDs (i.e., labels) $\mathcal{L}$ based on their similarity in terms of event attendance.


% \subsection{Event Segmentation} % (fold)
% \label{ssub:event_segmentation}

% As defined in \sect\ref{ssub:event}, an event is denoted as $e$. We assume a collection of $n$ images $\{x_i \in X\}_{i=1}^n$ are collected by one or more smart cameras, which contain the cropped face images of users. These will have wide variability, e.g., different views, poses, scales and illumination. Let $\{l_j \in L\}_{j=1}^m$ be a set of $m$ WiFi MAC addresses, i.e., $m$ people of interest (POI) to recognize. 

% Assuming after data collection, we have images $\{x_i \in X\}_{i=1}^n$ spanning multiple events, e.g., over the period of several days. {\sysname} segments images into $|E|$ subsets, namely the number of events. An image subset $\{x_{e_k, i} \in X_{e_k}\}$ in event $e_k$ is determined by the captured time and camera location. For instance, any images captured during the timeslot of event $e_k$, e.g, 14:00-15:00 on the 1st of May, by cameras in a particular room, are put into the image subset $X_{e_k}$. All the images in the same subset share the same event index. It is worth noting that one subject could have multiple face images in $\{x_{e_k, i} \in X_{e_k}\}$, e.g., captured at different lighting conditions or viewing angles. On the other hand, by inspecting the sniffed MAC addresses, we can also maintain an $m$-dimensional attendance observation vector $I_{e_k}^{\tau}$ for each event. $I_{e_k}^{\tau}[j]$ which is set to $1$ only if the user $j$'s MAC address $l_j \in L$ is detected in the event $e_k$. We refer readers to Fig.~\ref{fig:event_def} to see the examples of such event attachments. Due to the uncertain nature of WiFi sensing, the initial attendance observation $I_{e_k}^{\tau}$ is noisy and should be iteratively updated. These event attachments build \textit{coarse-grained} correlations between a set of face images and a set of device IDs, through their shared event $e_k$. However, at this stage the fine-grained mapping between an image $x_{e_k, i}$ and a MAC address $l_{e_k, j}$ is unknown. Note that, in the following sections, we use the superscript $\tau$ to denote the $\tau$-th iteration of those variables which will be updated in {\sysname}.

% \begin{figure}[t]\centering
% \includegraphics[width=0.75\columnwidth]{fig/i-clustering.pdf}  
% \caption{Cross-modality clustering. The final similarity is jointly determined by attendance assistance derived from event logs and similarity of features transformed via $f_{\theta}$, see Equ.~\ref{equ:id-ass_sim}. Detailed explanations can be found in \sect\ref{ssub:identity_assisted_clustering}.} 
% \label{fig:i-clustering}
% \end{figure}

\subsection{Cross-modality Clustering} % (fold)
\label{sub:cross_modality_clustering}

\noindent \textbf{Heterogeneous Features}. 
Given a pre-trained face representation model $f_{\theta}$, an image $x_i$ can be translated to the feature vector $\mathbf{z}_i$. Unlike conventional clustering that merely depends on the face feature similarity, {\sysname} merges face images \textit{across events} into a cluster (potentially belonging to the same subject) by incorporating attendance information as well. Recall that device attendance already reveals the identities of subjects (in the form of MAC addresses) in a particular event, and the captured images in the same event may contain the faces of these subjects as well. Despite the noise in observations, the overlapped subjects in different events can be employed as a prior that guides the image clustering. For example, if there are no shared MAC addresses sniffed in two events, then it is very likely that the face images captured in these two events should lie in different clusters. Formally, for an event $e_i$, we denote a device attendance vector as $\mathbf{u}_{k} = (u_k^1, u_k^2, \ldots, u_k^m)$, where $u_k^j=1$ if device $l_j$ is detected in event $e_k$. In this way, we could construct a heterogeneous feature $\widetilde{\mathbf{z}}_i = [\mathbf{z}_i, \mathbf{u}_{k}]$ for an image $x_i$ collected in the event $e_k$. Note that, as all images captured in a same event have the same attendance vector, this device attendance part are essentially enforced on cross-event image comparison. 

\noindent \textbf{Face Image Similarity}.
Given an image $x_i$ captured in event $e_k$ (i.e., $\widetilde{\mathbf{z}}_i = [\mathbf{z}_i, \mathbf{u}_{k}]$) and an image $x_j$ captured in event $e_p$ (i.e., $\widetilde{\mathbf{z}}_j = [\mathbf{z}_j, \mathbf{u}_{p}]$), the likelihood that two cross-event face images belong to the same subject is conditioned on two factors: i) the similarity of their feature representation between $\mathbf{z}_{i}$ and $\mathbf{z}_{j}$; and ii) the overlap ratio between the attendance observations in their corresponding events $\mathbf{u}_{k}$ and $\mathbf{u}_{p}$ respectively. The resulted joint similarity is a log likelihood $log(\mathbf{Pr}(x_i = x_j))$ defined as follows:

\begin{equation*}
\begin{split}
	\mathbf{Pr}(x_i = x_j) 
	& \propto \frac{exp(\beta * |\mathbf{u}_{k} \otimes \mathbf{u}_{p}|}{exp(\beta * |\mathbf{u}_{k} \oplus \mathbf{u}_{p}|)} * exp(-D(\mathbf{z}_i, \mathbf{z}_j)) \\
	log(\mathbf{Pr}(x_i = x_j)) & \propto \beta * \underbrace{(|\mathbf{u}_{k} \otimes \mathbf{u}_{p}| - |\mathbf{u}_{k} \oplus \mathbf{u}_{p}|)}_\text{attendance similarity} - \underbrace{D(\mathbf{z}_i, \mathbf{z}_j)}_\text{feature distance}
	\label{equ:id-ass_sim}
\end{split}
\end{equation*}

Here $\otimes$ and $\oplus$ are element-wise AND and OR, and $|\cdot|$ here is the $L^1$-norm. $z$ is the features transformed by the face representation model and $D$ is a distance measure between face features. $\beta$, analogous to the regularization parameter in composite loss functions, is a hyper-parameter that controls the contributions of the attendance assistance and feature similarity. The above derivation is inspired by the Jaccard coefficients, with the difference lying in the log function. The rationale behind the term $|\mathbf{u}_{k} \oplus \mathbf{u}_{p}|$ is that the more different subjects attending events, the more uncertain that any two images drawn across these events will point to the same subject. In contrast, when the intersection $|\mathbf{u}_{k} \otimes \mathbf{u}_{p}|$ is significant enough, the chance that these two images point to the same subject will become higher. This joint similarity can also be explained from a Bayesian perspective. The attendance similarity of two events can serve as a prior that two cross-event images belong to the same subject and the feature similarity can be seen as the likelihood. Together they determine the posterior probability that two cross-event images fall into the same cluster. Based on the above joint similarity, images across events are grouped into clusters $\mathcal{C} = \{c_i|i =1,2, \ldots, g\}$. We will soon discuss how to determine the number of clusters $g$ based on the complete set of MAC addresses $\mathcal{L}$ in the next section.

\begin{figure}[t]\centering
\includegraphics[width=\columnwidth]{fig/event_vector.pdf}  
\caption{Event vectors of an image cluster $c_i$ and device ID $l_j$. The $k$th element of the vector $r_{c_i}^k$ is set to $1$ only if it contains images attached with the event $e_k$. The event vector $\mathbf{r}_{l_j}$ of the device ID $l_j$ is similarly developed. This insight leads to Eq.~\ref{eq:assoc}.} 
\label{fig:event_vector}
\end{figure}

\subsection{Cluster Labeling} % (fold)
\label{sub:cluster_labeling}

\noindent \textbf{Fine-grained ID Association}.
After clustering, an image cluster is linked with multiple events that are associated with its member images. Naturally, we introduce an event vector $\mathbf{r}_{c_i} = (r_{c_i}^1, r_{c_i}^2, \ldots, r_{c_i}^{h})$ for for an image cluster $c_i$, where $h$ is the total number of events. $r_{c_i}^k$ is set to 1 only if $c_i$ contains images from event $e_k$. Fig.~\ref{fig:event_vector} shows an example of how an event vector is developed. Similarly, for a device ID $l_j$, its corresponding event vector $\mathbf{r}_{l_j} = (r_{l_j}^1, r_{l_j}^2, \ldots, r_{l_j}^h)$ can be determined by inspecting its occurrences in all WiFi sniffing observations. $r_{l_j}^k$ is set to $1$ only if the device ID (MAC address) $l_j$ is detected in the event $e_k$. The intuition behind ID association is that a device and a face image cluster of the same subject should share the most consistent attendance pattern in events, reflected by the similarity of their event vectors. Based on this intuition, {\sysname} assigns clusters with device IDs based on the matching level of their event vectors. Formally, a matching problem of bipartite graph can be formulated as follows:
\begin{equation}\label{eq:assoc}
	\begin{split}
		& \mathcal{L}_A = \sum_{ij} a_{ij} (\mathbf{r}_{c_i} - \mathbf{r}_{l_j})^2 \\
		 & \sum_{1 \leq j \leq m}  a_{ij} = 1, \quad \forall i \in \{1, \ldots, g\}
	\end{split}
\end{equation}
where the solution of the binary variable $a_{ij}$ assigns a device ID to a cluster. We note that when $m<g$, {\sysname} adds dummy nodes to create the complete bipartite graph. Then the complete bipartite graph problem can be solved by the Hungarian algorithm \cite{jonker1986improving}.

\begin{figure*}[t]
	\centering
	\begin{subfigure}{0.25\textwidth}
	\includegraphics[width=0.9\linewidth]{fig/eval/tsne/50/2018-04-02-114759_tnse.pdf}
	\caption{Pre-trained Model} \label{fig:tnse_pretrain}
	\end{subfigure}\hspace*{\fill}
	\begin{subfigure}{0.25\textwidth}
	\includegraphics[width=0.9\linewidth]{fig/eval/tsne/50/2018-05-05-13-23-29_tnse.pdf}
	\caption{1st iteration}
	\end{subfigure}\hspace*{\fill}
	\centering
	\begin{subfigure}{0.25\textwidth}
	\includegraphics[width=0.9\linewidth]{fig/eval/tsne/50/2018-05-06-06-04-50_tnse.pdf}
	\caption{2nd iteration} 
	\end{subfigure}\hspace*{\fill}
	\begin{subfigure}{0.25\textwidth}
	\includegraphics[width=0.9\linewidth]{fig/eval/tsne/50/2018-05-05-15-14-23_tnse.pdf}
	\caption{3rd iteration} 
	\end{subfigure}

\caption{An example of visual model update (\sect\ref{sub:visual_model_update}) in {\sysname} with a six-subject subset. Note that the pre-trained model in Fig.~\ref{fig:tnse_pretrain} has a narrow convex hull (black lines), clusters are dispersed and there is mis-classification (see false$\_3$ in Fig.~\ref{fig:tnse_pretrain}) as the pre-trained features are not discriminative enough to differentiate unseen subjects in a new environments. Over time, clusters become more compact and move further away from each other, leading to purer clustering results.} \label{fig:model_update}
\end{figure*}

\noindent \textbf{Probabilistic Labeling via Soft Voting}.
We now obtain the association between face images and device IDs. However, in practice, the number of clusters $g$ can vary due to the captured face images outside the POI, e.g., face images of short-term visitors. The choice of $g$ has a significant impact on the performance of clustering \cite{fraley1998many} which could further affect the following fine-tuning performance. To cope with this issue, {\sysname} sets the number of clusters $g$ greater than the number of POI $m$. With a larger number of clusters, although there are some unused clusters of non-POI after clustering, the association step will sieve them and only choose the most consistent $m$ clusters with the event logs of $m$ device IDs. Lastly, for every image, its assigned ID is finalized by decision voting on the individual association results computed with different $g$, which will be soon introduced in the next paragraph. Typically, a majority voting procedure would give a hard ID label for an image and use these $<$Image, ID$>$ pairs as training data to update the face representation model. However, due to the noise in device presence observations and errors in clustering, there will be mis-labeling in the training data that may confuse the model update. To account for the uncertainty of ID assignment, we adopt soft labels for voting. Then instead of voting for the most likely ID $y_i$ for an image $x_i$, we introduce a probability vector $\mathbf{y}_{i} = (y_{i,1}, y_{i,2}, \ldots, y_{i,m})$. Specifically, every image is associated with all POI and its associated soft label is derived by the votes for the subjects divided by the total number of votes. In this way, the soft label of each image is a valid probability distribution that sums up to 1. For instance, $y_{i,j}=0.4$ means that there are $40\%$ associations assigning the ID $j$ to the image $i$. Moreover, the soft labeled data $<x_i, \mathbf{y}_{i}>$ is compatible with the computation of cross-entropy. 

\noindent \textbf{Number of Clusters}.
We are now in a position to describe how to select the number of clusters $g$. We observed that, with a proper clustering algorithm (i.e., agglomerative clustering in our choice), non-POI's images will form separate small clusters but they will not be chosen in our follow-up association step. This is because that the number of devices ID $m$ is always less than the number of clusters ($g \in [2*m, 5*m]$), and only those images clusters with the most consistent event attendances are associated. The small clusters of outlier images often have scatted attendance vector and will be ignored in association. Therefore, soft voting with varying number of clusters can reinforce the core images of POI by giving large probability and assigns non-POI's images with small probability.


% \begin{figure}[t!]
% 	\centering
% 	\begin{subfigure}{0.32\textwidth}
% 	\includegraphics[width=\linewidth]{fig/eval/wifi_cm/nobar/no_start.pdf}
% 	\caption{Initial WiFi Attendance \emph{Obser.} } 
% 	\end{subfigure}\hspace*{\fill}
% 	\begin{subfigure}{0.32\textwidth}
% 	\includegraphics[width=\linewidth]{fig/eval/wifi_cm/nobar/no_cycle_8.pdf}
% 	\caption{Attendance \emph{Obser.} after 1st iter.} 
% 	\end{subfigure}\hspace*{\fill}
% 	\begin{subfigure}{0.36\textwidth}
% 	\includegraphics[width=\linewidth]{fig/eval/wifi_cm/bar/bar_cycle_15.pdf}
% 	\caption{Attendance \emph{Obser.} after 3rd iter.}
% 	\end{subfigure}

% 	\medskip
% 	\centering
% 	\begin{subfigure}{0.32\textwidth}
% 	\includegraphics[width=\linewidth]{fig/eval/wifi_cm/nobar/no_diff.pdf}
% 	\caption{Initial Attendance \emph{Errors}} 
% 	\end{subfigure}\hspace*{\fill}
% 	\begin{subfigure}{0.32\textwidth}
% 	\includegraphics[width=\linewidth]{fig/eval/wifi_cm/nobar/no_diff_cycle_6.pdf}
% 	\caption{Attendance \emph{Errors} after 1st iter.}
% 	\end{subfigure}\hspace*{\fill}
% 	\begin{subfigure}{0.36\textwidth}
% 	\includegraphics[width=\linewidth]{fig/eval/wifi_cm/bar/bar_diff_cycle_15.pdf}
% 	\caption{Attendance \emph{Errors} after 3rd iter.}
% 	\end{subfigure}

% \caption{An example of user attendance update (\sect\ref{ssub:id_update}) in {\sysname}, a 15-subject subset of $20$ events. \textbf{Top}: Attendance observations in events; \textbf{Bottom}: (absolute) errors of attendance observations in events. It can be seen that the IDs in events are gradually corrected as the model updates in {\sysname}.} \label{fig:id_update}
% \end{figure}


==> section/implementation.tex <==
%!TEX root = ../autotune.tex
\section{Implementation} % (fold)
\label{sec:implementation}
In this section, we introduce the implementation details of {\sysname} (code available at \url{https://github.com/Wayfear/Autotune}).

\subsection{Heterogeneous Data Sensing} % (fold)
\label{sub:heterogeneous_data_sensing}
% {\sysname} automatically labels face images cropped from surveillance cameras by leveraging sniffed WiFi signals. Therefore there are two modules in our data collection system, a face extraction module and a WiFi sniffing module \footnote{The study has received ethical approval XXX [no name for blind review]}.

\noindent \textbf{Face Extraction}.
This module consists of a front-end remote camera and a back-end computation server~\footnote{The study has received ethical approval R50950}. Specifically, the remote cameras in our experiment are diverse and include \emph{GoPro Hero 4}\footnote{\url{https://shop.gopro.com/cameras}}, \emph{Mi Smart Camera}\footnote{\url{https://www.mi.com/us/mj-panorama-camera/}} and \emph{Raspberry Pi Camera}\footnote{\url{https://www.raspberrypi.org/products/camera-module-v2/}}). We modified these cameras so that they are able to communicate and transfer data to the back-end through a wireless network. To avoid capturing excess data without people in it, we consider a motion-triggered mechnism with a circular buffer. It works by continuously taking low-resolution images, and comparing them to one another for changes caused by something moving in the camera's field of view. When a change is detected, the camera takes a higher-resolution video for $5$ seconds and reverts to low resolution capturing. All the collected videos are sent to the backend at every midnight. On the backend, a cascaded convolutional network based face detection module \cite{zhang2016joint} is used to drop videos with no face in them. The cropped faces from the remaining videos are supplied to {\sysname}.

\noindent \textbf{WiFi Sniffing}.
This module is realized on a WiFi-enabled laptop running Ubuntu 14.04. Our sniffer uses Aircrack-ng \footnote{\url{https://www.aircrack-ng.org/}} and tshark \footnote{\url{https://www.wireshark.org/docs/man-pages/tshark.html}} to opportunistically capture the WiFi packets in the vicinity. The captured packet has unencrypted information such as transmission time, source MAC address and the Received Signal Strengths (RSS). As {\sysname} aims to label face images for POI, our WiFi sniffer only records the packets containing MAC addresses of POI's and discards them otherwise, so as to not harvest addresses from people who have not given consent. A channel hop mechanism is used in the sniffing module to cope with cases where the POI's device(s) may connect to different WiFi networks, namely, on different wireless channels. The channel hop mechanism forces the sniffing channel to change by every second and monitor the active channels periodically (1 second) in the environment. The RSS value in the packet implies how far away the sniffed device is from the sniffer \cite{lu2016robust,lu2016elm}. By putting the sniffer near the camera, we can use a threshold to filter out those devices with low RSS values, e.g., less than -55 dBm in this work, as they are empirically unlikely to be within the camera's field of view.

\noindent \textbf{Event Segmentation}.
Depending on the context, the duration of events can be variable. However, for simplicity we use fix-duration events in this work. Specifically, we split a day into 12 intervals, each of which is $2$ hours long. We then discard those events that have neither face images nor sniffed MAC addresses of POI. 


\subsection{Face Recognition Model} % (fold)
\label{sub:face_recognition_model}
The face recogonition model used in {\sysname} is the state-of-the-art FaceNet \cite{schroff2015facenet}.

\noindent \textbf{Pre-training}.
FaceNet adopts the Inception-ResNet-v1 \cite{szegedy2017inception} as its backbone and its weights are pre-trained on the VGGFace2 dataset \cite{cao2017vggface2}. This dataset contains $3.31$ million
images of $9131$ subjects, with an average of $362.6$ images for each subject. Images are downloaded from Google Image Search and have large variations in pose, age, illumination, ethnicity and profession.
Pre-training is supervised by the triplet loss \cite{cheng2016person} and the training protocols, e.g, parameter settings, can be found in \cite{schroff2015facenet}. We found that the learnt face representation by FaceNet is generalizable and it is able to achieve an accuracy of 99.65\% on the LFW face verification task \footnote{\url{http://vis-www.cs.umass.edu/lfw/}}. Note that, FaceNet \cite{schroff2015facenet} not only learns a powerful recognition model but gives a very discriminative feature representation that can be used for clustering.

\noindent \textbf{Fine-tuning by \sysname}. The fine-tuning process has been explained in \sect\ref{sub:visual_model_update}, and here we provide some key implementation detials. After each round of label association (see \sect\ref{sub:cluster_labeling}), the labeled data is split into a training set and validation set, with a ratio of $8:2$ respectively. The pre-trained FaceNet is then fine-tuned on the training set, and the model that achieves the best performance on the validation set is saved. Note that the fine-tuning process in {\sysname} does not involve the test set. The online testing is performed on a held-out set that is collected on different days. To enhance the generalization ability, we use dropout training for regularization \cite{wager2013dropout}. The dropout ratio is set to $0.2$. We set the batch size to $50$ and one fine-tuning takes $100$ epochs. 

\subsection{System Configuration} % (fold)
\label{sub:parameter_configuration}

\noindent \textbf{Face Detection}.
As discussed in \sect\ref{sub:heterogeneous_data_sensing}, we use a cascaded convolution network to detect faces in videos. It is cascaded by three sub-networks, a proposal network, a refine network and an output network. Each of them can output bounding boxes of potential faces and the corresponding detection probabilities, i.e., confidences. Face detection with small confidence will be discarded early in the process and not sent to the next sub-network. In this work, the confidence threshold is set to $0.7$, $0.7$ and $0.9$ for three sub-networks respectively. Following the original setting in \cite{zhang2016joint}, we set the minimal face size in detection to $40 \times 40$ pixels.

\noindent \textbf{Setup of Face Clustering}.
In \sect\ref{sub:cross_modality_clustering}, we use a clustering algorithm to merge the images across events. Specifically, the clustering algorithm used in {\sysname} is agglomerative clustering \cite{beeferman2000agglomerative}, which is a method that recursively merges the pair of clusters that minimally increases a given linkage distance. The similarity metric adopted here is Euclidean distance. A linkage criterion determines which distance to use between sets of data points. In {\sysname}, this linkage criterion is set to the average distances of all sample pairs from two sets. \chris{As introduced in Sec.~\ref{sub:cluster_labeling}, the number of clusters $g$ is determined by the number of POI $m$. We vary $g$ from $2*m$ to $5*m$ and proceed soft voting, to account for the extra clusters of non-POI's face images and ambiguous/outlier images of POI.}

% \noindent \textbf{Threshold of Convergence}.
% The convergence of {\sysname} depends on when the residual of ID predictions in two iterations are below a certain threshold $\xi$ (see Algorithm.~\ref{alg:autotune}). $\xi$ affects the convergence speed, however, we fix it to $0.01$ to control the variables in the following evaluations. In practice, we observe that {\sysname} can work comparably for a relatively wide range of $\xi$.
% subsubsection threshold_of_convergence (end)

==> section/model_update.tex <==
%!TEX root = ../autotune.tex
\section{Model Updates} % (fold)
\label{sec:model_update}
We are now in a position to introduce the model update in {\sysname}. At every iteration, {\sysname} updates the last-iteration face representation model $f_{\theta}^{\tau}$ to $f_{\theta}^{\tau+1}$, by taking the labeled images as inputs. To correct the device observation errors, {\sysname} leverages these label images to update device attendance vector to $\mathbf{u}^{\tau}$ for all events. 

\subsection{Visual Model Update} % (fold)
\label{sub:visual_model_update}
\noindent \textbf{Discriminative Face Representation Learning}.
Face representation learning optimizes a representation loss $\mathcal{L}_R$ to enforce the learnt features as discriminative as possible. Strong discrimination bears two properties: inter-class dispersion and intra-class compactness. Inter-class dispersion pushes face images of different subjects away from one another and the intra-class compactness pulls the face images of the same subject together. Both of the properties are critical to face recognition. At iteration $\tau$, given the current labels $y_i^{\tau}$ for the $i$th face image $x_i$ and the transformed features $\mathbf{z}_i^{\tau} = f_{\theta}^{\tau}(x_i)$, the representation loss $\mathcal{L}_R$ is determined by a composition of softmax loss and center loss:
\begin{equation}
	\begin{split}
		\mathcal{L}_R &= \mathcal{L}_{softmax} + \mathcal{L}_{center} \\
				      &= \underbrace{\sum_{i}-log(\frac{e^{W_{y_i^{\tau}}^T\mathbf{z}_i^{\tau} + \mathbf{b}_{y_i^{\tau}}}}{\sum_{j=1}^{m}e^{W_{l_j}^T\mathbf{z}_i^{\tau} + \mathbf{b}_{l_j}}})}_\text{softmax loss} + \underbrace{\sum_{i}\frac{\lambda}{2} ||\mathbf{z}_i^{\tau} - \mathbf{o}_{y_i^{\tau}}||^2}_\text{center loss}
	\end{split}
	\label{equ:model_loss}
\end{equation}
where $W$ and $b$ are the weights and bias parameters in the last fully connected layer of the pre-trained model. $\mathbf{o}_{y_i^{\tau}}$ denotes a centroid feature vectors by averaging all feature vectors with the same identity label $y_i$. 
The center loss $\mathcal{L}_{center}$ explicitly enhances the intra-class compactness while the inter-class dispersion is implicitly strengthened by the softmax loss $\mathcal{L}_{softmax}$ \cite{wen2016discriminative}. $\lambda$ is a hyper-parameter that balances the above sub-losses. 

\noindent \textbf{Stochastic Center Loss}
The center loss $\mathcal{L}_{center}$ in Eq.~\ref{equ:model_loss} is shown to be helpful to enhance the intra-class compactness \cite{wen2016discriminative}. However, we cannot directly adopt it for fine-tuning as computing the centers requires explicit labels (see Eq.~\ref{equ:model_loss}) of images, while the association steps above only provide probabilistic ones through soft labels. To solve this, we propose a new loss called \emph{stochastic center loss} $\mathcal{L}_{stoc}$ to replace the center loss. Similar to the idea of fuzzy sets \cite{xie1991validity}, we allow each face image to belong to more than one subject. The membership grades indicate the degree to which an image belongs to each subject and can be directly retrieved from the soft labels and the stochastic center $\mathbf{o}_k^{\tau}$ for the $k$-th identity is given as:

\begin{equation}
	\mathbf{o}_k^{\tau} = \frac{\sum_i^{n}\mathbf{z}_i^{\tau} * y_{i,k}^{\tau}}{\sum_i^{n} y_{i,k}^{\tau}}
	\label{equ:fuzzy_center}
\end{equation}
This gives the stochastic center loss as follows:
\begin{equation}
\mathcal{L}_{stoc} = \sum_{i}\sum_{k} y_{i,k}^{\tau} *||\mathbf{z}_i^{\tau} - \mathbf{o}_k^{\tau}||^2
\end{equation}

We leave the softmax loss $\mathcal{L}_{softmax}$ the same as in Eq.~\ref{equ:model_loss}, because the soft labels are compatible with the computation of cross-entropy. The new representation loss to minimize is:
\begin{equation}
	\mathcal{L}_R = \mathcal{L}_{softmax} + \mathcal{L}_{stoc}
\end{equation}
{\sysname} updates the model parameters $\theta^{\tau}$ to $\theta^{\tau+1}$ based on the gradients of $\nabla_{\theta}\mathcal{L}_R$, which are calculated via back prorogation of errors. Compared with the dataset used for pre-training, which is usually in the order of millions \cite{cao2017vggface2}, the data used for fine-tuning is much smaller (several thousands). The mis-match between the small training data and the complex model architecture could result in overfitting. To prevent overfitting, we use the dropout mechanism in training, which is widely adopted to avoid overfitting \cite{lecun2015deep}. Meanwhile, as observed in \cite{hinton2015distilling,reed2014training}, the soft label itself can play the role of a regularizer, and make the trained model robust to noise and reduce overfitting. Fig.~\ref{fig:model_update} illustrates the effect of model update.

\subsection{User Attendance Update} % (fold)
\label{sub:user_attendance_update}
The device presence observations by WiFi sniffing are noisy because the WiFi signal of a device is opportunistic and people do not carry/use theirs devices all the time. Based on the results of the cluster labelling step introduced in \sect\ref{sub:cluster_labeling}, we have the opportunity to update our belief on which users attended each event. The update mechanism is as follows: Each image is associated with a user probability vector, whose elements denote the probability that the image correspondences to a particular user. By averaging the user probability vectors of all images that have been drawn from the same event ${e_k}$, and normalizing the result, we can estimate the user attendance of this event. The elements of the resulting user attendance vector $\widehat{\mathbf{u}}_k^{\tau}$ denote the probabilities of different users attending event $e_k$. 

We can now use $\widehat{\mathbf{u}}_k^{\tau}$ as a correction to update our previous wifi attendance vector $\mathbf{u}_{k}^{\tau}$  as follows:

\begin{equation}
	\mathbf{u}^{\tau+1}_{k} = \mathbf{u}^{\tau}_{k} - \gamma \cdot (\mathbf{u}^{\tau}_{k} - \widehat{\mathbf{u}}_k^{\tau})
\end{equation}
where $\gamma$ is a pre-defined parameter that controls the ID update rate. In principle, a large update rate will speed up the convergence rate, at the risk of missing the optima. {\sysname} sequentially repeats the above steps of clustering, labelling and model updates, until the changes $\xi$ in the user attendance model are negligible ($\leq 0.01$ in our case). Algorithm.~\ref{alg:autotune} summarizes the workflow.

\begin{algorithm2e}[t] 
\KwIn{pre-trained model $f_{\theta}^{1}$, images $\mathcal{X}$, POI's device IDs $\mathcal{L}$, threshold $\xi$}
\KwOut{adapted model $f_{\theta}^{\ast}$, corrected attendance observations $I^{\ast}$, soft image labels $Y^{\ast}$} 
\kwInit{Given sniffed $\mathcal{L}$ in all events $\mathcal{E}$, compute attendance vector $\mathbf{u}^0$}
$\tau=1$ \\
\While{$\sqrt{\frac{1}{h}\sum_{k=1}^{h}||\mathbf{u}^{(\tau)}_{k} - \mathbf{u}^{(\tau-1)}_{k}||^2} > \xi$}{
	$\mathcal{Z}^\tau = f_{\theta}^{\tau}(\mathcal{X})$ \Comment{feature transformation}\\
	\For{$g \leftarrow 2*m$ to $5*m$}{
	 	$\mathcal{C}^\tau \leftarrow$ \texttt{cross\_modality\_clustering}($\mathcal{Z}^\tau$, $\mathbf{u}^\tau$, g) \Comment{\sect\ref{sub:cross_modality_clustering}}\; 
	 	$A^\tau_g \leftarrow$ \texttt{cluster\_labeling}($\mathcal{C}^\tau$, $\mathbf{r}_c^\tau$, $\mathbf{r}_l^\tau$) \Comment{\sect\ref{sub:cluster_labeling}}\; 
	}
	$\mathcal{Y}^{\tau} \leftarrow$ \texttt{soft\_voting}($A^\tau$) \Comment{\sect\ref{sub:cluster_labeling}}\;
 	$\mathbf{o}^{\tau} \leftarrow$ \texttt{stochastic\_center}($\mathcal{Y}^{\tau}$, $\mathcal{Z}^\tau$) \Comment{\sect\ref{sub:visual_model_update}}\; 
 	$f_\theta^{\tau+1} \leftarrow$ \texttt{visual\_model\_update}($\mathcal{X}$, $\mathcal{Y}^\tau$, $\mathbf{o}^{\tau}$, $f_\theta^{\tau}$) \Comment{\sect\ref{sub:visual_model_update}} \;
 	$\mathbf{u}^{\tau+1} \leftarrow$ \texttt{user\_attendance\_update}($\mathcal{Y}^{\tau}$, $\mathbf{u}^{\tau}$) \Comment{\sect\ref{sub:user_attendance_update}} \;
  $\tau \leftarrow \tau + 1$
 }
% \nl \bf Pass\;
    \caption{{\bf {\sysname}} \label{alg:autotune}}

\end{algorithm2e}



==> section/overview_old.tex <==
%!TEX root = ../autotune.tex
\section{{\sysname} Overview} % (fold)
\label{sec:overview}

\begin{figure*}[ht]
	\begin{minipage}[b]{0.49\linewidth}
		\centering
		\includegraphics[width=\textwidth]{fig/event_def.pdf}
		\caption{An illustrative example of \emph{events} and showing their linked \emph{observations}. An \emph{event} is uniquely determined by spatial-temporal attributes and its participants. An event is also linked with two types of observations. Face observation are images cropped from surveillance videos and device observation are sniffed MAC address of participants' devices.}
		\label{fig:event_def}
	\end{minipage}
	\hfill
	\begin{minipage}[b]{0.49\linewidth}
		\centering
		\includegraphics[width=\textwidth]{fig/autotune_arch_v2.pdf}
		\caption{Workflow of {\sysname}. {\sysname} consists of 5 steps i) Heterogeneous Data Sensing ii) Cross-Modality Clustering iii) Cluster Labeling iv) Visual Model Update v) User Attendance Update. {\sysname} sequentially repeats the above five steps until the changes in the user attendance are negligible.}
		\label{fig:architecture}
	\end{minipage}
\end{figure*}

\subsection{System Model} % (fold)
\label{sub:system_model}
We consider a face recognition problem with $m$ people of interest (POI) and each subject owns one WiFi-enabled device, e.g., a smartphone. We denote the identity set as $\mathcal{Y} = \{y_j|j=1,2, \ldots, m\}$. The set of observed POI's devices in a particular environment is denoted by $\mathcal{L} = \{l_j|j=1,2, \ldots, m\}$, e.g., a set of MAC addresses. We assume the mapping from device MAC addresses $\mathcal{L}$ to the user identity $\mathcal{I}$ is known. A collection of face images $\mathcal{X} = \{x_j|j=1,2, \ldots, n\}$ is cropped from the surveillance videos in the same environment. Note that, to mimic the real-world complexity, our collection includes the faces of both POI and some non-POI, e.g., subjects with unknown device MAC addresses. We then assign face and device observations to different subsets based on their belonging events $\mathcal{E} = \{e_j|j=1,2, \ldots, h\}$. An event $e_j$ is the setting in which people interact with each other in a specific part of the environment for a given time interval. It is uniquely identified by three attributes: effective timeslot, location, and participants. Fig.~\ref{fig:event_def} demonstrates a few examples of events. Lastly, we also have a deep face representation model $f_{\theta}$ pre-trained on public datasets that contains no POI. Such model is trained with metric losses, e.g., triplet loss so that the learned features could bear a good property for clustering \cite{schroff2015facenet}.

In this sense, the problem addressed by {\sysname} is assigning IDs to images from noisy observations of images and WiFi MAC addresses, and using such learned ID-image associations to tune the pre-trained deep face representation model automatically.
% subsection system_model (end)

\subsection{System Architecture} % (fold)
\label{sub:system_architecture}
\sysname is based on two key observations: i) although collected by different modalities, both face images and device MAC addresses are linked with the identities of users who attend certain events; and ii) the tasks of model tuning and face-identity association should not be dealt with separately, but rather progress in tandem. Based on the above insights, {\sysname} works as follows (see Fig~\ref{fig:architecture}):
\begin{itemize}
	\item \emph{Heterogeneous Data Sensing}. This module collects facial and WiFi data (device attendance observations) through surveillance cameras and WiFi sniffers\footnote{\url{https://www.wireshark.org/}} in a target environment. Given the face images and sniffed WiFi MAC addresses, {\sysname} first segments them into events based on the time and location they were captured.

	\item \emph{Cross-modality Labeling}. This module first clusters face images based on their appearance similarity computed by the face representation model, and also taking into account information on device attendance in events. Each image cluster should broadly correspond to a user, and the cluster's images are drawn from a set of events. We then assign each cluster to the user whose device has been detected in as similar as possible set of events. 

	\item \emph{Model Updates}. Once images are labeled with user identity labels, this module then fine-tunes the pre-trained face representation model. {\sysname} further uses the cluster labels to update our belief on which device (MAC address) has participated in each event. 
\end{itemize}

The sensing module is one-off and we will detail its implementation in \sect\ref{sub:heterogeneous_data_sensing}. Labeling and model update modules are iteratively repeated until the changes in the user attendance model become negligible. The tuned model derived in the last iteration is regarded as the one best adapted to POI recognition in the new environment.




==> section/preliminaries.tex <==
%!TEX root = ../autotune.tex
\section{Preliminaries} % (fold)
\label{sec:preliminaries}

\begin{figure}[t]\centering
\includegraphics[width=\columnwidth]{fig/event_def.pdf}  
\caption{An illustrative example of \emph{events} and showing their linked face and device \emph{observations}. An \emph{event} is uniquely determined by spatial-temporal attributes and its participants. An event is also linked with two types of observations. The face observation are images cropped from surveillance videos and the device observation are sniffed MAC address of participants' devices.}
\label{fig:event_def}
\end{figure}

\subsection{Key Terms} % (fold)
\label{sub:key_terms}
In this section, we introduce some key terms and background that pave the way for \sect\ref{sec:autotune_solution}. 

\noindent \textbf{Event}:
As we will soon discuss in the next section, a key concept in {\sysname} is that of an \emph{event}. An event $e \in E$ is the setting in which people interact with each other in a specific part of the environment for a given time interval. It is uniquely identified by three attributes: effective timeslot, location, and participants. Fig.~\ref{fig:event_def} demonstrates a few examples of events. As we can see, an instance of an event might be a meeting in a conference room, exercise in a gym, or a lunch in the canteen. The spatio-temporal attributes of an event, i.e., timeslot and location, can either be obtained by side channel information (e.g. calendar), or for simplicity, they can be assumed to be fixed size cubes. However, the participants of an event, especially if it happens in a public space, are difficult to directly obtain. Details about how we create events in real-word experiments will be introduced in \sect\ref{ssub:event_duration}.

% \begin{definition}{(\textbf{Event})}
% An event $e \in E$ is the setting that subjects interact with entities in an environment for a time interval. It is uniquely identified by three attributes: effective timeslot, happening location, and involved (subject) identities. 
% \end{definition}
\noindent \textbf{observations}:
A smart camera and a WiFi sniffer are assumed to sense the identities in an environment. With the rapid development of camera systems and increasing deployment of WiFi access points, our assumption is practical. With these two sensor modalities, two types of observations can be attached to an event: i) cropped face images detected by the cameras, and ii) device observations (MAC addresses) which give weak user attendance or presence information through WiFi sniffing. Fig.~\ref{fig:event_def} illustrates the relationship between identity observations and events through examples.

\noindent \textbf{Pre-trained Model}:
A pre-trained model is used to transform the face images into discriminative features or representations, thereby aiding accurate clustering or classification. In this work, a deep neural network (DNN) for discriminative face representation is trained by a model provider, e.g., Facebook or Google, who are able to access a large number of annotated face images. This model needs to be fine-tuned by smart-cameras in a particular space or environment, e.g., images acquired from an office or home. Note that our formulation does not require access to the images used for pre-training, just the weights and architecture of the pre-trained network model. 

\subsection{Challenges and Objectives} % (fold)
\label{sub:challenges_and_objectives}
{\sysname} is motived by the fact that, neither of the above sensor observations can \emph{directly} provide \emph{accurate} identity information. Face images are strong biometrics, but they cannot directly convey identity information without external labels i.e. a recognition model is needed to transfer biometrics to actual identity. The pre-trained model is no exception here. Given the mapping between MAC address and user identity, device observations are able to provide unique and direct identity information. In practice, the mapping between a MAC address to a user is easy to get for cameras in smart spaces. In order to authenticate legitimate WiFi users, say Eduroam \footnote{https://en.wikipedia.org/wiki/Eduroam}, device MAC addresses and user account information are bound together. However, device observations are usually noisy because a detected MAC address does not necessarily indicate that the device owner is co-located. Therefore, the objectives of {\sysname} are two-fold: i) automatically label face images that have noisy observations; and ii) reliably adapt the pre-trained model to recognize the faces of users in new environments.
% subsection notations (end)

==> section/problem.tex <==
%!TEX root = ../autotune.tex
\section{Problem Statement} % (fold)
\label{sec:problem_statement}

\begin{figure}[t]\centering
\includegraphics[width=\columnwidth]{fig/event_def.pdf}  
\caption{An illustrative example of \emph{event} and its face and WiFi \emph{observations}. \chris{will complete the caption}}
\label{fig:intuition}
\end{figure}


\subsection{Preliminaries} % (fold)
\label{sub:preliminaries}
\subsubsection{Background} % (fold)
\label{ssub:background}
Initially, a deep neural network (DNN) for discriminative face representation is trained by a model provider, e.g., Facebook or Google, who are able to access a large amount of annotated face images. We refer to this pre-trained model as the \emph{donor model} and it needs to be fine-tuned by smart-cameras in a particular space or environment, e.g., images acquired from an office or home. Note that our formulation does not require access to the images used for pre-training, just the weights and architecture of the pre-trained model. In addition to the donor model, a smart camera environment also possesses two types of data: i) cropped face images detected by the cameras, and ii) device observations (MAC addresses) which give weak presence information through WiFi sniffing. 

\subsubsection{Challenges and Objectives} % (fold)
\label{ssub:challenges_and_objectives}
Face images are strong biometrics, but they cannot directly convey identity information without external labels i.e. a recognition model is needed to transfer biometrics to actual identity. Given the mapping between MAC address and user identity, device observations are able to provide unique and direct identity information. In practice, the mapping between a MAC address to a user is easy to get for cameras in smart spaces. In order to authenticate legitimate WiFi users, say Eduroam \footnote{https://en.wikipedia.org/wiki/Eduroam}, device MAC addresses and user account information are bound together. However, device observations are usually noisy because a detected MAC address does not necessarily indicate that the device owner is co-located. Therefore, the objectives of AutoTune are two-fold: i) automatically label face images that have noisy observations; and ii) reliably adapt the donor model to recognize the faces of users in new environments.

\subsubsection{Key Terms} % (fold)
\label{ssub:key_terms}
 We assume a collection of $n$ images $\{x_i \in X\}_{i=1}^n$ are collected by one or more smart cameras, which contains the cropped face images of users. These will have wide variability e.g. different views, poses, scales and illumination. Let $\{l_j \in L\}_{j=1}^m$ be a set of $m$ WiFi MAC addresses, i.e., $m$ people of interest (POI) to recognize. The instance-level labels $\{y_i^{\tau} \in L\}_{i=1}^n$ match the identities to the face images $\{x_i \in X\}_{i=1}^n$ at iteration $\tau$. With the updated model $f_{\theta}^{\tau}$, a face image $x_i$ is transformed to a feature representation $\{z_i^{\tau} \in Z\}_{i=1}^n$. After $T$ iterations, the resultant model is denoted as $f_{\theta}^T$. 

\subsection{Problem Formulation} % (fold)
\label{sub:problem_formulation}
AutoTune adapts the donor model by iteratively minimizing two losses in tandem: i) the face representation loss $\mathcal{L}_R$ and ii) the identity association loss $\mathcal{L}_A$, which will now be discussed in turn.
\subsubsection{Representation Loss} % (fold)
\label{ssub:representation_loss}
The representation loss $\mathcal{L}_R$ reflects how discriminative the learned face features are. Strong discrimination bears two properties: inter-class dispersion and intra-class compactness. Inter-class dispersion pushes face images of different subjects away from one another and the intra-class compactness pulls the face images of the same subject together. Both of these steps are critical to face recognition. At iteration $\tau$, given the current labels $y_i^{\tau}$ for the $i$th face image $x_i$ and the transformed features $z_i^{\tau} = f_{\theta}^{\tau}(x_i)$, the representation loss $\mathcal{L}_R$ is determined by a composition of softmax loss and center loss:

\begin{equation}
	\begin{split}
		\mathcal{L}_R &= \mathcal{L}_{softmax} + \mathcal{L}_{center} \\
				      &= \underbrace{\sum_{i}-log(\frac{e^{W_{y_i^{\tau}}^Tz_i^{\tau} + b_{y_i^{\tau}}}}{\sum_{j=1}^{m}e^{W_{l_j}^Tz_i^{\tau} + b_{l_j}}})}_\text{softmax loss} + \underbrace{\sum_{i}\frac{\lambda}{2} ||z_i^{\tau} - c_{y_i^{\tau}}||^2}_\text{center loss}
	\end{split}
	\label{equ:model_loss}
\end{equation}
where $W$ and $b$ are the weights and bias parameters in the last fully connected layer of the pre-trained model. The center loss $\mathcal{L}_{center}$ explicitly enhances the intra-class compactness while the inter-class dispersion is implicitly strengthened by the softmax loss $\mathcal{L}_{softmax}$ \cite{wen2016discriminative}. $\lambda$ is a hyper-parameter that balances the above sub-losses. 

\subsubsection{Association Loss} % (fold)
\label{ssub:association_loss}
The association loss $\mathcal{L}_A$ measures how accurately the device ID is assigned to the face images. At iteration $\tau$, the ID assignment is a linear programming problem:
\begin{equation}
	\begin{split}
		& \mathcal{L}_A = \sum_{ij} a_{ij}^{\tau} \varepsilon_{ij}^{\tau} \\
		 \sum_{1 \leq j \leq m} & a_{ij}^{\tau} = 1, \quad \forall i \in \{1, \ldots, n\}
	\end{split}
	\label{equ:loss}
\end{equation}
where $a_{ij}^{\tau}$ is a binary variable that is set to $1$ if the face image is assigned to identity label $j$, and $0$ otherwise. The parameter is $\varepsilon_{ij}^{\tau}$ is the cost of such an assignment and will be discussed in detail in \sect\ref{ssub:fine_grained_id_association}. As we can see, the association loss is also constrained to guarantee that exactly one identity label is given to an image, but not vice versa. Through minimizing the the association loss $\mathcal{L}_A$, the label $y_i^{\tau+1}$ of an image can be derived by the optimal assignment of $a_{ij}^{\tau}$ at iteration $\tau$.                                                                                                                                    
% At a high level, the optimization of the total losses goes as follows. At the first iteration $\tau=0$, the face images $X$ are grouped into clusters $G^{0}$, based on the similarity of their transformed features $Z^{0}$ using the donor model $f_{\theta}^{0}$. The clusters of face images are then associated with the device MAC addresses, to achieve the minimum association costs of $\mathcal{L}_A$. The cost $\varepsilon_{ij}$ of association will be shortly introduced in the next section. Images in the same cluster then share the same assigned identity label $Y^0$. The labels assigned in the association step, will be leveraged to fine-tune the representation model $f_{\theta}^{0}$. Above association and fine-tuning steps completes one iteration. The optimization keep perform such iterations, until converges. The model $f_{\theta}^{T}$ derived in the last iteration (t=T) is taken as the final model adapted to the new environment. 




==> section/solution.tex <==
%!TEX root = ../autotune.tex
\section{AutoTune Solution} % (fold)
\label{sec:autotune_solution}
\begin{figure}[t]\centering
\includegraphics[width=0.99\columnwidth]{fig/autotune_arch_v2.pdf}  
\caption{Workflow of {\sysname}. {\sysname} consists of 5 steps i) Event segmentation ii) Cross-Modality clustering iii) Cluster Labeling iv) Visual Model Update v) User Attendance Update. {\sysname} sequentially repeats the above five steps until the changes in the user attendance model are negligible.}
\label{fig:architecture}
\end{figure}

% \subsection{Event Segmentation} % (fold)
% \label{ssub:event_segmentation}

% As defined in \sect\ref{ssub:event}, an event is denoted as $e$. We assume a collection of $n$ images $\{x_i \in X\}_{i=1}^n$ are collected by one or more smart cameras, which contain the cropped face images of users. These will have wide variability, e.g., different views, poses, scales and illumination. Let $\{l_j \in L\}_{j=1}^m$ be a set of $m$ WiFi MAC addresses, i.e., $m$ people of interest (POI) to recognize. 

% Assuming after data collection, we have images $\{x_i \in X\}_{i=1}^n$ spanning multiple events, e.g., over the period of several days. {\sysname} segments images into $|E|$ subsets, namely the number of events. An image subset $\{x_{e_k, i} \in X_{e_k}\}$ in event $e_k$ is determined by the captured time and camera location. For instance, any images captured during the timeslot of event $e_k$, e.g, 14:00-15:00 on the 1st of May, by cameras in a particular room, are put into the image subset $X_{e_k}$. All the images in the same subset share the same event index. It is worth noting that one subject could have multiple face images in $\{x_{e_k, i} \in X_{e_k}\}$, e.g., captured at different lighting conditions or viewing angles. On the other hand, by inspecting the sniffed MAC addresses, we can also maintain an $m$-dimensional attendance observation vector $I_{e_k}^{\tau}$ for each event. $I_{e_k}^{\tau}[j]$ which is set to $1$ only if the user $j$'s MAC address $l_j \in L$ is detected in the event $e_k$. We refer readers to Fig.~\ref{fig:event_def} to see the examples of such event attachments. Due to the uncertain nature of WiFi sensing, the initial attendance observation $I_{e_k}^{\tau}$ is noisy and should be iteratively updated. These event attachments build \textit{coarse-grained} correlations between a set of face images and a set of device IDs, through their shared event $e_k$. However, at this stage the fine-grained mapping between an image $x_{e_k, i}$ and a MAC address $l_{e_k, j}$ is unknown. Note that, in the following sections, we use the superscript $\tau$ to denote the $\tau$-th iteration of those variables which will be updated in {\sysname}.

% \begin{figure}[t]\centering
% \includegraphics[width=0.75\columnwidth]{fig/i-clustering.pdf}  
% \caption{Cross-modality clustering. The final similarity is jointly determined by attendance assistance derived from event logs and similarity of features transformed via $f_{\theta}$, see Equ.~\ref{equ:id-ass_sim}. Detailed explanations can be found in \sect\ref{ssub:identity_assisted_clustering}.} 
% \label{fig:i-clustering}
% \end{figure}

\subsection{Cross-modality Clustering} % (fold)
\label{ssub:identity_assisted_clustering}
Before assigning fine-grained ID labels, {\sysname} needs to cluster images across events. Unlike conventional clustering that merely depends on the feature similarity, {\sysname} merges face images \textit{across events} into a cluster (potentially belonging to the same subject) by incorporating attendance information as well. Recall that the attendance observation vector $I_{e_k}^{\tau}$ already reveals the identities of subjects (in the form of MAC addresses) in the event $e_k$, and the captured images $X_{e_k}$ may contain the faces of these subjects. Despite the noise in observations, the overlapped subjects in different events can be employed as a prior that guides the image clustering. For example, if there are no shared MAC addresses sniffed in two events, then it is very likely that the face images captured in these two events should lie in different clusters. 

Formally, the likelihood that two cross-event face images $x_{e_k, i}$ and $x_{e_p, j}$ belong to the same subject is conditioned on two factors: i) the similarity of their feature representation between $z_{e_k, i}^{\tau}$ and $z_{e_p, j}^{\tau}$; and ii) the overlap ratio between the attendance observations in their corresponding events. The resulted joint similarity is a log likelihood $log(\mathbf{Pr}(y_{e_k, i}^{\tau} = y_{e_p, j}^{\tau}))$ defined as follows:

\begin{equation}
\begin{split}
	\mathbf{Pr}(y_{e_k, i}^{\tau} = y_{e_p, j}^{\tau}) 
	& \propto \frac{exp(\beta * |I_{e_k}^\tau \otimes I_{e_p}^\tau|)}{exp(\beta * |I_{e_k}^\tau \oplus I_{e_p}^\tau|)} * exp(-D(z_{e_k, i}^{\tau}, z_{e_p, j}^{\tau})) \\
	log(\mathbf{Pr}(y_{e_k, i}^{\tau} = y_{e_p, j}^{\tau})) & \propto \beta * \underbrace{(|I_{e_k}^\tau \otimes I_{e_p}^\tau| - |I_{e_k}^\tau \oplus I_{e_p}^\tau|)}_\text{attendance assistance} - \underbrace{D(z_{e_k, i}^{\tau}, z_{e_p, j}^{\tau})}_\text{feature distance}
	\label{equ:id-ass_sim}
\end{split}
\end{equation}

Here $\otimes$ and $\oplus$ are element-wise AND and OR, and $|\cdot|$ here is the $L^1$-norm. $z$ is the features transformed by the face representation model and $D$ is a distance measure between face features. $\beta$, \chris{analogous to the regularization parameter in composite loss functions,} is a hyper-parameter that controls the contributions of the attendance assistance and feature similarity. Fig.~\ref{fig:i-clustering} demonstrates how the joint similarity between two cross-event images is determined. The above derivation is inspired by the Jaccard coefficients, with the difference lying in the log function. The rationale behind the term $|I_{e_k} \oplus I_{e_p}|$ is that the more different subjects attending events, the more uncertain that any two images drawn across these events will point to the same subject. In contrast, when the intersection $|I_{e_k} \otimes I_{e_p}|$ is significant enough, the chance that these two images point to the same subject will become higher. \chris{Equ.~\ref{equ:id-ass_sim} can also be explained from a Bayesian perspective. The attendance similarity of two events can serve as a prior that two cross-event images belong to the same subject and the feature similarity can be seen as the likelihood. Together they determine the posterior probability that two cross-event images fall into the same cluster.} Based on the above joint similarity, images across events are grouped into $g$ clusters. We will soon discuss how to determine $g$ based on the complete set of MAC addresses $\{l_j \in L\}_{j=1}^m$ in \sect\ref{ssub:voting}.

\begin{figure}[t]\centering
\includegraphics[width=0.99\columnwidth]{fig/event_vector.pdf}  
\caption{Event vectors of an image cluster and device ID. The $k$th element of the vector $V_{G_i}[k]$ is set to $1$ only it contains images attached with the event $e_k$. The event vector $V_{l_j}$ of the device ID $l_j$ is similarly developed. See \sect\ref{sub:cross_modality_labeling} for more details.} 
\label{fig:event_vector}
\end{figure}

\subsection{Cluster Labeling} % (fold)
\label{sub:cross_modality_labeling}
\subsubsection{Fine-grained ID Association} % (fold)
\label{ssub:fine_grained_id_association}
After clustering, an image cluster is linked with multiple events that are associated with its member images. We introduce an event vector $V_{G_i}^{\tau}$ for an image cluster $G_i$, with $V_{G_i}^{\tau}[k]$ that is set to 1 only if it contains images attached with the event $e_k$. The length of the event vector is determined by the number of events $|E|$. Fig.~\ref{fig:event_vector} shows an example of how an event vector is developed. Similarly, for a device ID $l_j$, its corresponding event vector $V_{l_j}^{\tau}$ can be determined by inspecting its occurrences in all user attendance observations. $V_{l_j}^{\tau}[k]$ is set to $1$ only if the device ID (MAC address) $l_j$ is detected in the event $e_k$. \chris{The intuition behind ID association is that the device and the face image cluster of the same subject should share the most consistent attendance pattern in events, reflected by the similarity of their event vectors. Based on this intuition, {\sysname} assigns cluster $G_i$ with device IDs based on the matching level of their event vectors.} Formally, a matching problem of bipartite graph can be formulated as follows:
\begin{equation}
	\begin{split}
		& \mathcal{L}_A = \sum_{ij} a_{ij}^{\tau} (V_{G_i}^{\tau} - V_{l_j}^{\tau})^2 \\
		 & \sum_{1 \leq j \leq m}  a_{ij}^{\tau} = 1, \quad \forall i \in \{1, \ldots, g\}
	\end{split}
\end{equation}
where the solution of the binary variable $a_{ij}^{\tau}$ assigns a device ID to a cluster, and the images in a cluster are labeled by the same assigned ID. We note that when $m<g$, {\sysname} adds dummy nodes to create the complete bipartite graph. Then the complete bipartite graph problem can be solved by the Hungarian algorithm \cite{jonker1986improving}.

\subsubsection{\chris{Probabilistic Labeling via Soft Voting}} % (fold)
\label{ssub:voting}
We now obtain the instance-level ID association. However, in practice, the number of clusters $g$ can vary due to the captured face images outside the POI, e.g., face images of short-term visitors. The choice of $g$ has a significant impact on the performance of clustering \cite{fraley1998many} which could further affect the following fine-tuning performance. To include the non-POI, the number of clusters $g$ should be greater than the number of POI $m$, but the exact number of $g$ is impossible to know beforehand. To bypass this issue, we set the cluster number $g$, from $2*m$ to $5*m$ and run the clustering (\sect\ref{ssub:identity_assisted_clustering}) and association (\sect\ref{ssub:fine_grained_id_association}) for multiple rounds. {\sysname} is robust to extra clusters of non-POI, when $g$ is greater than $m$. Although there are some unused clusters of non-POI after clustering, the association step will sieve them and only choose the most consistent $m$ clusters with the event logs of $m$ device IDs. Lastly, for every image, its assigned ID is finalized by decision voting on the individual association results computed with different $g$, ranging from $2*m$ to $5*m$.

Typically, a majority voting procedure would give a hard ID label for an image and use these $<$Image, ID$>$ pairs as training data to update the face representation model. However, due to the noise in device presence observations and errors in clustering, there will be mis-labeling in the training data that may confuse the model update. To account for the uncertainty of ID assignment, we adopt soft labels for voting. More specifically, instead of voting for the most likely ID $y_i^{\tau}$ for an image $x_i$, we introduce a normalized vector $m$-dimension $\mathbf{y}_{i}^{\tau}$. \chris{Specifically, every image is associated with all POI and its associated soft label is derived by the votes for the subjects divided by the total number of votes. In this way, the soft label of each image is a valid probability distribution that sums up to 1.} For instance, $\mathbf{y}_{i}^{\tau}[j]=0.4$ means that there are $40\%$ associations assigning the ID $j$ to the image $i$. Moreover, the soft labeled data $<x_i, \mathbf{y}_{i}^{\tau}>$ is compatible with the computation of cross-entropy. \chris{  Besides coping the uncertain number of non-POI, soft voting can actually handle the feature uncertainty issue of outliers. Outliers of POI refer to those images belongs to a POI but very dissimilar to the majority. Those images can significantly confuse the clustering process. We observed that, with a proper clustering algorithm (i.e., agglomerative clustering in our choice), outlier images will form separate small clusters but they will not be chosen in our follow-up association step. This is because that the number of devices ID $m$ is always less than the number of clusters ($[2*m, 5*m]$), and only those images clusters with the most consistent event attendances are associated. The small clusters of outlier images often have scatted attendance vector and will be ignored in association. Therefore, soft voting with varying number of clusters can reinforce the core images of POI by giving large probability and assigns outlier images with very small probability.
} 

% \begin{figure}[t!]
% 	\centering
% 	\begin{subfigure}{0.32\textwidth}
% 	\includegraphics[width=\linewidth]{fig/eval/wifi_cm/nobar/no_start.pdf}
% 	\caption{Initial WiFi Attendance \emph{Obser.} } 
% 	\end{subfigure}\hspace*{\fill}
% 	\begin{subfigure}{0.32\textwidth}
% 	\includegraphics[width=\linewidth]{fig/eval/wifi_cm/nobar/no_cycle_8.pdf}
% 	\caption{Attendance \emph{Obser.} after 1st iter.} 
% 	\end{subfigure}\hspace*{\fill}
% 	\begin{subfigure}{0.36\textwidth}
% 	\includegraphics[width=\linewidth]{fig/eval/wifi_cm/bar/bar_cycle_15.pdf}
% 	\caption{Attendance \emph{Obser.} after 3rd iter.}
% 	\end{subfigure}

% 	\medskip
% 	\centering
% 	\begin{subfigure}{0.32\textwidth}
% 	\includegraphics[width=\linewidth]{fig/eval/wifi_cm/nobar/no_diff.pdf}
% 	\caption{Initial Attendance \emph{Errors}} 
% 	\end{subfigure}\hspace*{\fill}
% 	\begin{subfigure}{0.32\textwidth}
% 	\includegraphics[width=\linewidth]{fig/eval/wifi_cm/nobar/no_diff_cycle_6.pdf}
% 	\caption{Attendance \emph{Errors} after 1st iter.}
% 	\end{subfigure}\hspace*{\fill}
% 	\begin{subfigure}{0.36\textwidth}
% 	\includegraphics[width=\linewidth]{fig/eval/wifi_cm/bar/bar_diff_cycle_15.pdf}
% 	\caption{Attendance \emph{Errors} after 3rd iter.}
% 	\end{subfigure}

% \caption{An example of user attendance update (\sect\ref{ssub:id_update}) in {\sysname}, a 15-subject subset of $20$ events. \textbf{Top}: Attendance observations in events; \textbf{Bottom}: (absolute) errors of attendance observations in events. It can be seen that the IDs in events are gradually corrected as the model updates in {\sysname}.} \label{fig:id_update}
% \end{figure}

\subsection{Visual Model Update} % (fold)
\label{sub:model_update}
We are now in a position to introduce the model update in {\sysname}. By taking the labeled data as inputs, the face representation model $f_{\theta}^{\tau}$ updates its weights and biases $\theta$ to $f_{\theta}^{\tau+1}$. 

\subsubsection{Discriminative Face Representation} % (fold)
\label{ssub:discriminative_face_repre}
Face representation learning optimizes a representation loss $\mathcal{L}_R$ to force the learnt features as discriminative as possible. Strong discrimination bears two properties: inter-class dispersion and intra-class compactness. Inter-class dispersion pushes face images of different subjects away from one another and the intra-class compactness pulls the face images of the same subject together. Both of the properties are critical to face recognition. At iteration $\tau$, given the current labels $y_i^{\tau}$ for the $i$th face image $x_i$ and the transformed features $z_i^{\tau} = f_{\theta}^{\tau}(x_i)$, the representation loss $\mathcal{L}_R$ is determined by a composition of softmax loss and center loss:
\begin{equation}
	\begin{split}
		\mathcal{L}_R &= \mathcal{L}_{softmax} + \mathcal{L}_{center} \\
				      &= \underbrace{\sum_{i}-log(\frac{e^{W_{y_i^{\tau}}^Tz_i^{\tau} + b_{y_i^{\tau}}}}{\sum_{j=1}^{m}e^{W_{l_j}^Tz_i^{\tau} + b_{l_j}}})}_\text{softmax loss} + \underbrace{\sum_{i}\frac{\lambda}{2} ||z_i^{\tau} - c_{y_i^{\tau}}||^2}_\text{center loss}
	\end{split}
	\label{equ:model_loss}
\end{equation}
where $W$ and $b$ are the weights and bias parameters in the last fully connected layer of the pre-trained model. The center loss $\mathcal{L}_{center}$ explicitly enhances the intra-class compactness while the inter-class dispersion is implicitly strengthened by the softmax loss $\mathcal{L}_{softmax}$ \cite{wen2016discriminative}. $\lambda$ is a hyper-parameter that balances the above sub-losses. 

\subsubsection{Fuzzy Center Loss} % (fold)
\label{ssub:fuzzy_center_loss}
The center loss $\mathcal{L}_{center}$ in Equ.~\ref{equ:model_loss} is shown to be helpful to enhance the intra-class compactness \cite{wen2016discriminative}. However, we cannot directly adopt it for fine-tuning as computing the centers requires explicit labels (see Equ.~\ref{equ:model_loss}) of images, but the association steps above only provide probabilistic ones through soft labels. To solve this, we propose a new loss called \emph{stochastic center loss} $\mathcal{L}_{stoc}$ to replace the center loss. Similar to the core idea of fuzzy clustering \cite{xie1991validity}, we allow each face image to belong to more than one subject. In fact, the membership grades indicating the degree to which an image belongs to each subject can be directly retrieved from the soft labels and the stochastic center $\mathbf{o}_k^{\tau}$ is given as:

\begin{equation}
	\mathbf{o}_k^{\tau} = \frac{\sum_i^{n}\mathbf{z}_i^{\tau} * y_{i,k}^{\tau}}{\sum_i^{n} y_{i,k}^{\tau}}
	\label{equ:fuzzy_center}
\end{equation}
The fuzzifier $\eta$ is a hyper-parameter that determines the level of cluster fuzziness. A large $\eta$ results in smaller membership values and hence, fuzzier clusters. This gives the stochastic center loss as follows:
\begin{equation}
\mathcal{L}_{stoc} = \sum_{i}\sum_{k} \mathbf{y}_{i}^{\tau}[k]*||z_i^{\tau} - \mathbf{o}_k^{\tau}||^2
\end{equation}

\subsubsection{Fine-tuning} % (fold)
\label{ssub:fine_tuning}
We leave the softmax loss $\mathcal{L}_{softmax}$ the same as in Equ.~\ref{equ:model_loss}, because the soft labels are compatible with the computation of cross-entropy. The new representation loss to minimize is:
\begin{equation}
	\mathcal{L}_R = \mathcal{L}_{softmax} + \mathcal{L}_{stoc}
\end{equation}
{\sysname} updates the model parameters $\theta^{\tau}$ to $\theta^{\tau+1}$ based on the gradients of $\nabla_{\theta}\mathcal{L}_R$, which are calculated via back prorogation of errors. Compared with the dataset used for pre-training, which is usually in the order of millions \cite{cao2017vggface2}, the data used for fine-tuning is much smaller (several thousands). The mis-match between the small training data and the complex model architecture could result in overfitting. To prevent overfitting, we use the dropout mechanism in training, which is widely adopted to avoid overfitting \cite{lecun2015deep}. Meanwhile, as observed in \cite{hinton2015distilling,reed2014training}, the soft label itself can play the role of a regularizer, and make the trained model robust to noise and reduce overfitting.

\subsection{User Attendance Update} % (fold)
\label{ssub:id_update}
The device presence observations by WiFi sniffing are noisy because the WiFi signal of a device is opportunistic and people do not carry/use theirs devices all the time. Based on the results of the cluster labelling step introduce in \sect\ref{sub:cross_modality_labeling}, we have the opportunity to update our belief on which users attended each event. 

The update mechanism is as follows: Each image is associated with a user probability vector, whose elements denote the probability that the image correspondences to a particular user. By averaging the user probability vectors of all images that have been drawn from the same event ${e_k}$, and normalizing the result, we can estimate the user attendance of this event. The elements of the resulting user attendance vector $\hat{I}_{e_k}$ denote the probabilities of different users attending event ${e_k}$. 

We can now use $\hat{I}_{e_k}$ as a correction to update our previous wifi attendance vector $I_{e_k}^{\tau}$  as follows:

\begin{equation}
	I^{\tau+1}_{e_k} = I^{\tau}_{e_k} - \beta \cdot (I^{\tau}_{e_k} - \hat{I}_{e_k})
\end{equation}
where $\beta$ is a pre-defined parameter that controls the ID update rate. In principle, a large update rate will speed up the convergence rate, at the risk of missing the optima.

\begin{figure*}[t!]
	\centering
	\begin{subfigure}{0.2\textwidth}
	\includegraphics[width=\linewidth]{fig/eval/tsne/50/2018-04-02-114759_tnse.pdf}
	\caption{Pre-trained Model} \label{fig:tnse_pretrain}
	\end{subfigure}\hspace*{\fill}
	\begin{subfigure}{0.2\textwidth}
	\includegraphics[width=\linewidth]{fig/eval/tsne/50/2018-05-05-13-23-29_tnse.pdf}
	\caption{1st iteration}
	\end{subfigure}\hspace*{\fill}
	\centering
	\begin{subfigure}{0.2\textwidth}
	\includegraphics[width=\linewidth]{fig/eval/tsne/50/2018-05-06-06-04-50_tnse.pdf}
	\caption{2nd iteration} 
	\end{subfigure}\hspace*{\fill}
	\begin{subfigure}{0.2\textwidth}
	\includegraphics[width=\linewidth]{fig/eval/tsne/50/2018-05-05-15-14-23_tnse.pdf}
	\caption{3rd iteration} 
	\end{subfigure}

\caption{An example of visual model update (\sect\ref{sub:model_update}) in {\sysname} with a six subject subset. Note that the pre-trained model in Fig.~\ref{fig:tnse_pretrain} has a narrow convex hull (black lines), clusters are dispersed and there is misclassification. After the first iteration, clusters become more distinct and span more of the embedding space. Over time, clusters become more compact and move further away from each other, leading to purer clustering results.} \label{fig:model_update}
\end{figure*}

{\sysname} sequentially repeats the above steps of clustering, labelling and model updates, until the changes in the user attendance model are negligible. Algorithm.~\ref{alg:autotune} summarizes the workflow.

\begin{algorithm}[h] 
\KwIn{pre-trained model $f_{\theta}^{0}$, WiFi sniffed attendance observations $I^{0}$, images $X$, number of POI $m$, threshold $\xi$}
\KwOut{adapted model $f_{\theta}^{\ast}$, corrected attendance observations $I^{\ast}$, soft image labels $Y^{\ast}$} 
\kwInit{Segment attendance observations $I^0$ and images $X$ into subsets $I^0_{e_k}$ and $X_{e_k}$ based on events $E$ \Comment{\sect\ref{ssub:event_segmentation}}} 
$\tau=0$ \\
\While{$\sqrt{\frac{1}{|E|}\sum_{k=1}^{|E|}||I^{(\tau)}_{e_k} - I^{(\tau-1)}_{e_k}||^2} > \xi$}{
	$Z^\tau = f_{\theta}^{\tau}(X)$ \Comment{feature transformation}\\
	\For{$g \leftarrow m$ to $3*m$}{
	 	$G^\tau \leftarrow$ \texttt{cross\_modality\_clustering}($Z^\tau$, $I^\tau$, g) \Comment{\sect\ref{ssub:identity_assisted_clustering}}\; 
	 	$A^\tau_g \leftarrow$ \texttt{ID\_association}($G^\tau$, $I^\tau$) \Comment{\sect\ref{ssub:fine_grained_id_association}}\; 
	}
	$Y^{\tau} \leftarrow$ \texttt{voting}($A^\tau$) \Comment{\sect\ref{ssub:voting}}\;
 	$c^{\tau} \leftarrow$ \texttt{fuzzy\_center}($Y^{\tau}$, $Z^\tau$) \Comment{\sect\ref{ssub:fuzzy_center_loss}}\; 
 	$f_\theta^{\tau+1} \leftarrow$ \texttt{visual\_model\_update}($Y^\tau$, $c^\tau$, $f_\theta^{\tau}$, X) \Comment{\sect\ref{ssub:fine_tuning}} \;
 	$I^{\tau+1} \leftarrow$ \texttt{user\_attendance\_update}($Y^{\tau}$, $I^{\tau}$) \Comment{\sect\ref{ssub:id_update}} \;
  $\tau \leftarrow \tau + 1$
 }
% \nl \bf Pass\;
    \caption{{\bf {\sysname}} \label{alg:autotune}}

\end{algorithm}


